SURF: Improving classifiers in production by learning from busy and noisy end users

Supervised learning classifiers inevitably make mistakes in production, perhaps mis-labeling an email, or flagging an otherwise routine transaction as fraudulent. It is vital that the end users of such a system are provided with a means of relabeling data points that they deem to have been mislabeled. The classifier can then be retrained on the relabeled data points in the hope of performance improvement. To reduce noise in this feedback data, well known algorithms from the crowdsourcing literature can be employed. However, the feedback setting provides a new challenge: how do we know what to do in the case of user non-response? If a user provides us with no feedback on a label then it can be dangerous to assume they implicitly agree: a user can be busy, lazy, or no longer a user of the system! We show that conventional crowdsourcing algorithms struggle in this user feedback setting, and present a new algorithm, SURF, that can cope with this non-response ambiguity.

==> ICAIF_source_60 copy/thetable.tex <==
\scalebox{.47}{
\begin{tabular}{lllllllllllllllllllllllllllll}
\toprule
    & {} & \multicolumn{27}{l}{Acc} \\
    & $M$ & \multicolumn{9}{l}{5} & \multicolumn{9}{l}{10} & \multicolumn{9}{l}{15} \\
    & $p_c$ & \multicolumn{3}{l}{0.25} & \multicolumn{3}{l}{0.50} & \multicolumn{3}{l}{0.75} & \multicolumn{3}{l}{0.25} & \multicolumn{3}{l}{0.50} & \multicolumn{3}{l}{0.75} & \multicolumn{3}{l}{0.25} & \multicolumn{3}{l}{0.50} & \multicolumn{3}{l}{0.75} \\
    & $p_u$ &            0.25 &            0.50 &            0.75 &            0.25 &            0.50 &            0.75 &            0.25 &            0.50 &            0.75 &            0.25 &            0.50 &            0.75 &            0.25 &            0.50 &            0.75 &            0.25 &            0.50 &            0.75 &            0.25 &            0.50 &            0.75 &            0.25 &            0.50 &            0.75 &            0.25 &            0.50 &            0.75 \\
$\epsilon$ & Model &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 &                 \\
\midrule
0.0 & CATD &   0.987$\pm$0.0 &  0.746$\pm$0.02 &  0.743$\pm$0.02 &    0.98$\pm$0.0 &  0.824$\pm$0.01 &  0.494$\pm$0.02 &   0.974$\pm$0.0 &  0.791$\pm$0.02 &  0.356$\pm$0.03 &     1.0$\pm$0.0 &  0.959$\pm$0.01 &  0.751$\pm$0.01 &   0.999$\pm$0.0 &  0.948$\pm$0.01 &  0.571$\pm$0.07 &   0.999$\pm$0.0 &  0.938$\pm$0.01 &  0.499$\pm$0.03 &     1.0$\pm$0.0 &   0.991$\pm$0.0 &  0.756$\pm$0.02 &     1.0$\pm$0.0 &   0.988$\pm$0.0 &  0.664$\pm$0.06 &     1.0$\pm$0.0 &  0.986$\pm$0.01 &  0.594$\pm$0.04 \\
    & DS &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &   0.911$\pm$0.1 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 \\
    & EBCC &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.948$\pm$0.07 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.982$\pm$0.04 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 \\
    & GLAD &   0.986$\pm$0.0 &  0.898$\pm$0.01 &  0.692$\pm$0.04 &   0.979$\pm$0.0 &  0.821$\pm$0.01 &  0.461$\pm$0.04 &   0.974$\pm$0.0 &  0.797$\pm$0.01 &  0.314$\pm$0.02 &     1.0$\pm$0.0 &    0.97$\pm$0.0 &  0.683$\pm$0.13 &     1.0$\pm$0.0 &  0.948$\pm$0.01 &  0.505$\pm$0.05 &   0.999$\pm$0.0 &  0.938$\pm$0.01 &  0.386$\pm$0.02 &     1.0$\pm$0.0 &   0.993$\pm$0.0 &  0.758$\pm$0.11 &     1.0$\pm$0.0 &   0.989$\pm$0.0 &  0.497$\pm$0.05 &     1.0$\pm$0.0 &   0.985$\pm$0.0 &  0.432$\pm$0.03 \\
    & LFC &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.877$\pm$0.12 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.977$\pm$0.07 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &   0.97$\pm$0.06 \\
    & MV &   0.986$\pm$0.0 &  0.874$\pm$0.01 &  0.576$\pm$0.02 &  0.972$\pm$0.01 &  0.823$\pm$0.01 &  0.471$\pm$0.02 &  0.967$\pm$0.01 &   0.78$\pm$0.02 &  0.379$\pm$0.02 &   0.999$\pm$0.0 &  0.964$\pm$0.01 &  0.632$\pm$0.03 &   0.999$\pm$0.0 &  0.953$\pm$0.01 &  0.584$\pm$0.01 &     1.0$\pm$0.0 &  0.934$\pm$0.01 &  0.517$\pm$0.03 &     1.0$\pm$0.0 &    0.99$\pm$0.0 &  0.717$\pm$0.03 &     1.0$\pm$0.0 &    0.99$\pm$0.0 &  0.665$\pm$0.02 &     1.0$\pm$0.0 &  0.983$\pm$0.01 &  0.619$\pm$0.04 \\
    & SURF &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.941$\pm$0.11 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.688$\pm$0.26 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.991$\pm$0.03 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &   0.576$\pm$0.1 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &   0.95$\pm$0.08 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.972$\pm$0.06 \\
    & ZC &   0.986$\pm$0.0 &  0.898$\pm$0.01 &  0.744$\pm$0.02 &    0.98$\pm$0.0 &  0.822$\pm$0.01 &  0.503$\pm$0.02 &   0.975$\pm$0.0 &  0.796$\pm$0.01 &  0.292$\pm$0.02 &     1.0$\pm$0.0 &    0.97$\pm$0.0 &  0.761$\pm$0.03 &   0.999$\pm$0.0 &  0.948$\pm$0.01 &  0.566$\pm$0.03 &   0.999$\pm$0.0 &  0.938$\pm$0.01 &  0.392$\pm$0.08 &     1.0$\pm$0.0 &   0.993$\pm$0.0 &  0.803$\pm$0.03 &     1.0$\pm$0.0 &   0.988$\pm$0.0 &  0.598$\pm$0.09 &     1.0$\pm$0.0 &   0.986$\pm$0.0 &  0.426$\pm$0.09 \\
    & iBCC &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.935$\pm$0.09 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.981$\pm$0.04 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.972$\pm$0.06 \\
0.1 & CATD &   0.95$\pm$0.01 &  0.746$\pm$0.02 &  0.747$\pm$0.01 &  0.947$\pm$0.01 &  0.596$\pm$0.13 &  0.504$\pm$0.02 &   0.92$\pm$0.01 &   0.64$\pm$0.03 &  0.253$\pm$0.01 &    0.99$\pm$0.0 &  0.768$\pm$0.05 &  0.747$\pm$0.01 &    0.99$\pm$0.0 &  0.861$\pm$0.02 &  0.506$\pm$0.01 &   0.986$\pm$0.0 &   0.86$\pm$0.01 &   0.25$\pm$0.01 &   0.998$\pm$0.0 &  0.936$\pm$0.01 &  0.746$\pm$0.02 &   0.997$\pm$0.0 &  0.932$\pm$0.01 &  0.503$\pm$0.02 &   0.995$\pm$0.0 &  0.933$\pm$0.01 &  0.265$\pm$0.06 \\
    & DS &   0.991$\pm$0.0 &    0.99$\pm$0.0 &   0.992$\pm$0.0 &   0.995$\pm$0.0 &   0.993$\pm$0.0 &   0.994$\pm$0.0 &   0.995$\pm$0.0 &   0.992$\pm$0.0 &  0.762$\pm$0.17 &     1.0$\pm$0.0 &   0.999$\pm$0.0 &   0.999$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.939$\pm$0.09 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &   0.943$\pm$0.1 \\
    & EBCC &   0.993$\pm$0.0 &   0.991$\pm$0.0 &   0.994$\pm$0.0 &   0.994$\pm$0.0 &   0.993$\pm$0.0 &   0.996$\pm$0.0 &   0.995$\pm$0.0 &   0.992$\pm$0.0 &  0.841$\pm$0.13 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &   0.99$\pm$0.03 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.971$\pm$0.07 \\
    & GLAD &   0.95$\pm$0.01 &  0.857$\pm$0.01 &  0.706$\pm$0.01 &  0.933$\pm$0.01 &  0.734$\pm$0.01 &  0.521$\pm$0.01 &  0.906$\pm$0.01 &   0.67$\pm$0.02 &   0.33$\pm$0.01 &   0.988$\pm$0.0 &  0.933$\pm$0.01 &  0.756$\pm$0.01 &    0.99$\pm$0.0 &  0.861$\pm$0.02 &   0.57$\pm$0.02 &   0.986$\pm$0.0 &  0.865$\pm$0.01 &  0.362$\pm$0.01 &   0.998$\pm$0.0 &   0.96$\pm$0.01 &  0.779$\pm$0.02 &   0.997$\pm$0.0 &  0.932$\pm$0.01 &  0.585$\pm$0.02 &   0.995$\pm$0.0 &  0.931$\pm$0.01 &  0.379$\pm$0.02 \\
    & LFC &   0.991$\pm$0.0 &    0.99$\pm$0.0 &   0.992$\pm$0.0 &   0.994$\pm$0.0 &   0.993$\pm$0.0 &   0.993$\pm$0.0 &   0.996$\pm$0.0 &   0.992$\pm$0.0 &  0.765$\pm$0.18 &     1.0$\pm$0.0 &   0.999$\pm$0.0 &   0.999$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.933$\pm$0.09 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.959$\pm$0.09 \\
    & MV &  0.957$\pm$0.01 &  0.856$\pm$0.01 &  0.638$\pm$0.03 &   0.92$\pm$0.01 &  0.764$\pm$0.02 &  0.499$\pm$0.02 &  0.878$\pm$0.03 &  0.652$\pm$0.02 &  0.351$\pm$0.02 &   0.991$\pm$0.0 &   0.94$\pm$0.01 &  0.703$\pm$0.01 &   0.984$\pm$0.0 &  0.883$\pm$0.02 &  0.584$\pm$0.02 &  0.978$\pm$0.01 &  0.832$\pm$0.01 &  0.437$\pm$0.02 &   0.998$\pm$0.0 &   0.968$\pm$0.0 &  0.762$\pm$0.02 &   0.995$\pm$0.0 &  0.947$\pm$0.01 &  0.643$\pm$0.03 &   0.992$\pm$0.0 &   0.91$\pm$0.01 &  0.496$\pm$0.02 \\
    & SURF &   0.998$\pm$0.0 &   0.998$\pm$0.0 &   0.998$\pm$0.0 &   0.999$\pm$0.0 &   0.999$\pm$0.0 &   0.999$\pm$0.0 &   0.999$\pm$0.0 &   0.998$\pm$0.0 &  0.921$\pm$0.14 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.827$\pm$0.16 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.989$\pm$0.04 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &   0.999$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.618$\pm$0.16 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.928$\pm$0.14 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.991$\pm$0.03 \\
    & ZC &  0.953$\pm$0.01 &  0.857$\pm$0.01 &   0.75$\pm$0.01 &  0.948$\pm$0.01 &  0.734$\pm$0.01 &  0.517$\pm$0.02 &   0.92$\pm$0.01 &  0.676$\pm$0.02 &  0.282$\pm$0.01 &    0.99$\pm$0.0 &  0.933$\pm$0.01 &  0.757$\pm$0.01 &    0.99$\pm$0.0 &  0.863$\pm$0.02 &  0.542$\pm$0.01 &   0.986$\pm$0.0 &  0.864$\pm$0.01 &  0.317$\pm$0.02 &   0.998$\pm$0.0 &   0.96$\pm$0.01 &   0.77$\pm$0.02 &   0.997$\pm$0.0 &  0.932$\pm$0.01 &  0.561$\pm$0.02 &   0.995$\pm$0.0 &  0.933$\pm$0.01 &  0.361$\pm$0.03 \\
    & iBCC &   0.993$\pm$0.0 &   0.991$\pm$0.0 &   0.994$\pm$0.0 &   0.994$\pm$0.0 &   0.993$\pm$0.0 &   0.997$\pm$0.0 &   0.995$\pm$0.0 &   0.992$\pm$0.0 &  0.756$\pm$0.15 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.979$\pm$0.07 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.963$\pm$0.08 \\
0.2 & CATD &  0.806$\pm$0.07 &  0.758$\pm$0.02 &  0.747$\pm$0.02 &  0.862$\pm$0.01 &    0.5$\pm$0.01 &  0.504$\pm$0.01 &  0.819$\pm$0.02 &  0.251$\pm$0.01 &  0.246$\pm$0.01 &  0.958$\pm$0.01 &  0.751$\pm$0.01 &  0.746$\pm$0.01 &  0.942$\pm$0.01 &  0.593$\pm$0.12 &   0.49$\pm$0.01 &  0.924$\pm$0.01 &  0.626$\pm$0.01 &  0.246$\pm$0.02 &   0.979$\pm$0.0 &  0.751$\pm$0.01 &  0.747$\pm$0.01 &  0.973$\pm$0.01 &  0.802$\pm$0.01 &  0.498$\pm$0.02 &  0.952$\pm$0.01 &  0.721$\pm$0.03 &  0.248$\pm$0.01 \\
    & DS &  0.966$\pm$0.01 &  0.955$\pm$0.01 &  0.965$\pm$0.01 &  0.971$\pm$0.01 &  0.974$\pm$0.01 &  0.936$\pm$0.05 &  0.983$\pm$0.01 &   0.989$\pm$0.0 &  0.436$\pm$0.12 &   0.996$\pm$0.0 &   0.996$\pm$0.0 &   0.996$\pm$0.0 &   0.997$\pm$0.0 &   0.998$\pm$0.0 &  0.986$\pm$0.04 &   0.999$\pm$0.0 &     1.0$\pm$0.0 &  0.539$\pm$0.13 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &   0.999$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.996$\pm$0.01 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.525$\pm$0.13 \\
    & EBCC &  0.969$\pm$0.01 &  0.963$\pm$0.01 &  0.974$\pm$0.01 &  0.968$\pm$0.01 &  0.972$\pm$0.01 &  0.977$\pm$0.02 &  0.977$\pm$0.01 &   0.984$\pm$0.0 &  0.356$\pm$0.12 &   0.996$\pm$0.0 &   0.997$\pm$0.0 &   0.998$\pm$0.0 &   0.996$\pm$0.0 &   0.997$\pm$0.0 &   0.999$\pm$0.0 &   0.998$\pm$0.0 &   0.999$\pm$0.0 &   0.484$\pm$0.2 &   0.999$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &   0.999$\pm$0.0 &     1.0$\pm$0.0 &  0.987$\pm$0.02 &   0.999$\pm$0.0 &     1.0$\pm$0.0 &  0.477$\pm$0.15 \\
    & GLAD &  0.893$\pm$0.01 &   0.83$\pm$0.02 &  0.723$\pm$0.01 &  0.857$\pm$0.01 &  0.666$\pm$0.02 &  0.519$\pm$0.02 &  0.802$\pm$0.01 &  0.496$\pm$0.01 &  0.305$\pm$0.01 &  0.956$\pm$0.01 &  0.879$\pm$0.01 &  0.757$\pm$0.01 &  0.926$\pm$0.01 &  0.753$\pm$0.02 &  0.549$\pm$0.01 &  0.915$\pm$0.01 &  0.626$\pm$0.01 &  0.325$\pm$0.02 &   0.973$\pm$0.0 &  0.904$\pm$0.01 &  0.773$\pm$0.02 &  0.965$\pm$0.01 &  0.802$\pm$0.01 &  0.553$\pm$0.02 &   0.95$\pm$0.01 &   0.71$\pm$0.02 &  0.321$\pm$0.01 \\
    & LFC &  0.967$\pm$0.01 &  0.959$\pm$0.01 &  0.968$\pm$0.01 &  0.972$\pm$0.01 &  0.976$\pm$0.01 &  0.958$\pm$0.03 &  0.983$\pm$0.01 &    0.99$\pm$0.0 &  0.457$\pm$0.13 &   0.996$\pm$0.0 &   0.997$\pm$0.0 &   0.997$\pm$0.0 &   0.997$\pm$0.0 &   0.998$\pm$0.0 &   0.999$\pm$0.0 &   0.999$\pm$0.0 &     1.0$\pm$0.0 &  0.643$\pm$0.16 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.588$\pm$0.11 \\
    & MV &   0.92$\pm$0.01 &  0.836$\pm$0.02 &  0.675$\pm$0.02 &   0.85$\pm$0.01 &  0.705$\pm$0.02 &  0.504$\pm$0.01 &  0.773$\pm$0.01 &  0.564$\pm$0.03 &  0.324$\pm$0.01 &  0.966$\pm$0.01 &  0.894$\pm$0.01 &  0.742$\pm$0.01 &  0.919$\pm$0.01 &  0.783$\pm$0.02 &  0.552$\pm$0.02 &  0.894$\pm$0.01 &  0.675$\pm$0.02 &   0.37$\pm$0.03 &   0.979$\pm$0.0 &  0.918$\pm$0.01 &   0.77$\pm$0.02 &  0.961$\pm$0.01 &  0.827$\pm$0.01 &  0.585$\pm$0.01 &  0.941$\pm$0.01 &  0.761$\pm$0.01 &  0.387$\pm$0.02 \\
    & SURF &   0.995$\pm$0.0 &    0.99$\pm$0.0 &   0.989$\pm$0.0 &   0.993$\pm$0.0 &   0.994$\pm$0.0 &  0.973$\pm$0.02 &   0.993$\pm$0.0 &   0.991$\pm$0.0 &   0.71$\pm$0.09 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &   0.95$\pm$0.11 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.983$\pm$0.04 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &   0.74$\pm$0.22 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.909$\pm$0.12 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &   0.942$\pm$0.1 \\
    & ZC &  0.894$\pm$0.01 &  0.825$\pm$0.02 &  0.748$\pm$0.02 &  0.874$\pm$0.01 &  0.666$\pm$0.02 &   0.51$\pm$0.01 &  0.827$\pm$0.01 &  0.498$\pm$0.01 &  0.254$\pm$0.01 &  0.959$\pm$0.01 &  0.879$\pm$0.01 &  0.754$\pm$0.01 &  0.943$\pm$0.01 &  0.753$\pm$0.02 &  0.507$\pm$0.01 &  0.924$\pm$0.01 &  0.632$\pm$0.01 &  0.274$\pm$0.03 &   0.979$\pm$0.0 &  0.904$\pm$0.01 &  0.757$\pm$0.01 &  0.973$\pm$0.01 &  0.802$\pm$0.01 &  0.523$\pm$0.01 &  0.952$\pm$0.01 &  0.723$\pm$0.03 &  0.282$\pm$0.01 \\
    & iBCC &  0.969$\pm$0.01 &  0.963$\pm$0.01 &  0.974$\pm$0.01 &  0.968$\pm$0.01 &  0.973$\pm$0.01 &   0.96$\pm$0.05 &  0.978$\pm$0.01 &   0.985$\pm$0.0 &  0.366$\pm$0.15 &   0.996$\pm$0.0 &   0.996$\pm$0.0 &   0.998$\pm$0.0 &   0.996$\pm$0.0 &   0.997$\pm$0.0 &   0.999$\pm$0.0 &   0.998$\pm$0.0 &   0.999$\pm$0.0 &  0.574$\pm$0.13 &   0.999$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &   0.999$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &   0.999$\pm$0.0 &     1.0$\pm$0.0 &   0.58$\pm$0.11 \\
0.3 & CATD &  0.742$\pm$0.02 &  0.738$\pm$0.01 &  0.734$\pm$0.01 &   0.71$\pm$0.02 &  0.499$\pm$0.02 &  0.494$\pm$0.01 &  0.658$\pm$0.02 &  0.249$\pm$0.02 &  0.247$\pm$0.01 &   0.88$\pm$0.02 &  0.749$\pm$0.01 &  0.756$\pm$0.01 &  0.822$\pm$0.01 &  0.504$\pm$0.01 &  0.504$\pm$0.01 &  0.774$\pm$0.03 &  0.255$\pm$0.01 &  0.254$\pm$0.01 &  0.922$\pm$0.01 &  0.758$\pm$0.01 &  0.745$\pm$0.01 &  0.873$\pm$0.02 &  0.493$\pm$0.01 &  0.494$\pm$0.01 &  0.831$\pm$0.01 &  0.279$\pm$0.09 &  0.251$\pm$0.01 \\
    & DS &   0.92$\pm$0.01 &  0.896$\pm$0.02 &  0.884$\pm$0.01 &  0.905$\pm$0.03 &  0.825$\pm$0.05 &   0.69$\pm$0.05 &  0.952$\pm$0.02 &   0.54$\pm$0.12 &   0.406$\pm$0.1 &  0.981$\pm$0.01 &  0.972$\pm$0.01 &  0.918$\pm$0.03 &   0.99$\pm$0.01 &  0.982$\pm$0.02 &  0.736$\pm$0.08 &   0.996$\pm$0.0 &  0.761$\pm$0.12 &  0.295$\pm$0.13 &   0.996$\pm$0.0 &   0.996$\pm$0.0 &  0.944$\pm$0.03 &   0.998$\pm$0.0 &  0.989$\pm$0.02 &  0.732$\pm$0.07 &   0.999$\pm$0.0 &  0.812$\pm$0.12 &  0.327$\pm$0.13 \\
    & EBCC &  0.924$\pm$0.01 &  0.903$\pm$0.02 &  0.913$\pm$0.01 &    0.9$\pm$0.02 &  0.888$\pm$0.03 &  0.848$\pm$0.07 &  0.939$\pm$0.02 &  0.646$\pm$0.11 &  0.257$\pm$0.09 &  0.978$\pm$0.01 &   0.98$\pm$0.01 &  0.957$\pm$0.03 &  0.987$\pm$0.01 &   0.991$\pm$0.0 &  0.765$\pm$0.05 &  0.994$\pm$0.01 &   0.896$\pm$0.1 &   0.205$\pm$0.1 &   0.99$\pm$0.01 &  0.984$\pm$0.02 &  0.918$\pm$0.02 &   0.997$\pm$0.0 &  0.983$\pm$0.02 &  0.617$\pm$0.07 &   0.998$\pm$0.0 &  0.931$\pm$0.08 &  0.231$\pm$0.07 \\
    & GLAD &   0.85$\pm$0.01 &  0.791$\pm$0.01 &  0.723$\pm$0.01 &  0.723$\pm$0.02 &  0.604$\pm$0.02 &  0.507$\pm$0.01 &  0.671$\pm$0.02 &  0.414$\pm$0.02 &   0.28$\pm$0.02 &  0.893$\pm$0.01 &  0.819$\pm$0.01 &  0.759$\pm$0.01 &  0.792$\pm$0.01 &  0.645$\pm$0.01 &  0.527$\pm$0.01 &  0.748$\pm$0.03 &  0.478$\pm$0.02 &  0.297$\pm$0.01 &  0.922$\pm$0.01 &   0.84$\pm$0.01 &  0.755$\pm$0.01 &  0.838$\pm$0.02 &   0.67$\pm$0.01 &  0.521$\pm$0.01 &  0.815$\pm$0.01 &  0.506$\pm$0.01 &  0.292$\pm$0.01 \\
    & LFC &  0.924$\pm$0.01 &  0.906$\pm$0.02 &    0.9$\pm$0.02 &  0.913$\pm$0.03 &  0.873$\pm$0.03 &  0.739$\pm$0.06 &  0.955$\pm$0.02 &  0.579$\pm$0.13 &   0.427$\pm$0.1 &  0.982$\pm$0.01 &   0.98$\pm$0.01 &  0.972$\pm$0.02 &   0.99$\pm$0.01 &  0.992$\pm$0.01 &  0.873$\pm$0.09 &   0.996$\pm$0.0 &  0.944$\pm$0.09 &  0.371$\pm$0.16 &   0.996$\pm$0.0 &   0.996$\pm$0.0 &   0.999$\pm$0.0 &   0.998$\pm$0.0 &   0.999$\pm$0.0 &  0.874$\pm$0.12 &   0.999$\pm$0.0 &   0.97$\pm$0.06 &  0.405$\pm$0.15 \\
    & MV &   0.88$\pm$0.01 &  0.806$\pm$0.01 &  0.692$\pm$0.01 &  0.763$\pm$0.03 &  0.645$\pm$0.01 &  0.502$\pm$0.01 &  0.649$\pm$0.02 &  0.476$\pm$0.02 &  0.292$\pm$0.02 &  0.908$\pm$0.01 &  0.833$\pm$0.01 &  0.754$\pm$0.02 &  0.822$\pm$0.02 &  0.676$\pm$0.01 &  0.534$\pm$0.01 &  0.742$\pm$0.03 &   0.53$\pm$0.02 &  0.314$\pm$0.01 &  0.934$\pm$0.01 &  0.856$\pm$0.01 &  0.756$\pm$0.01 &  0.858$\pm$0.01 &  0.701$\pm$0.01 &  0.532$\pm$0.01 &  0.798$\pm$0.02 &  0.554$\pm$0.02 &  0.308$\pm$0.01 \\
    & SURF &   0.985$\pm$0.0 &  0.977$\pm$0.01 &  0.948$\pm$0.01 &   0.985$\pm$0.0 &  0.982$\pm$0.01 &  0.847$\pm$0.06 &  0.962$\pm$0.01 &  0.968$\pm$0.01 &  0.486$\pm$0.09 &   0.999$\pm$0.0 &     1.0$\pm$0.0 &  0.988$\pm$0.03 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.977$\pm$0.06 &   0.998$\pm$0.0 &   0.998$\pm$0.0 &   0.97$\pm$0.07 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.826$\pm$0.21 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.944$\pm$0.12 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &     1.0$\pm$0.0 \\
    & ZC &   0.85$\pm$0.01 &  0.784$\pm$0.01 &  0.735$\pm$0.01 &  0.736$\pm$0.02 &  0.602$\pm$0.02 &  0.495$\pm$0.01 &  0.683$\pm$0.03 &  0.413$\pm$0.02 &  0.252$\pm$0.02 &  0.893$\pm$0.01 &  0.814$\pm$0.01 &  0.758$\pm$0.01 &  0.824$\pm$0.01 &  0.645$\pm$0.01 &  0.508$\pm$0.01 &  0.779$\pm$0.03 &  0.477$\pm$0.02 &  0.259$\pm$0.01 &  0.923$\pm$0.01 &  0.838$\pm$0.01 &  0.746$\pm$0.01 &  0.875$\pm$0.01 &   0.67$\pm$0.01 &    0.5$\pm$0.01 &  0.832$\pm$0.01 &  0.505$\pm$0.01 &  0.258$\pm$0.01 \\
    & iBCC &  0.924$\pm$0.01 &  0.903$\pm$0.02 &  0.913$\pm$0.02 &  0.906$\pm$0.02 &  0.888$\pm$0.03 &   0.812$\pm$0.1 &  0.937$\pm$0.02 &  0.585$\pm$0.13 &  0.259$\pm$0.09 &  0.979$\pm$0.01 &  0.979$\pm$0.01 &  0.984$\pm$0.01 &  0.986$\pm$0.01 &   0.991$\pm$0.0 &  0.967$\pm$0.05 &  0.994$\pm$0.01 &  0.929$\pm$0.11 &   0.28$\pm$0.16 &   0.994$\pm$0.0 &   0.994$\pm$0.0 &   0.998$\pm$0.0 &   0.997$\pm$0.0 &   0.999$\pm$0.0 &  0.938$\pm$0.12 &   0.998$\pm$0.0 &  0.956$\pm$0.07 &  0.354$\pm$0.14 \\
0.4 & CATD &  0.751$\pm$0.02 &  0.744$\pm$0.02 &  0.744$\pm$0.01 &  0.496$\pm$0.02 &  0.496$\pm$0.02 &   0.49$\pm$0.01 &  0.248$\pm$0.02 &   0.25$\pm$0.01 &  0.257$\pm$0.01 &  0.752$\pm$0.01 &  0.758$\pm$0.01 &  0.758$\pm$0.02 &  0.557$\pm$0.08 &  0.505$\pm$0.02 &  0.506$\pm$0.01 &  0.516$\pm$0.02 &  0.254$\pm$0.01 &  0.247$\pm$0.01 &  0.752$\pm$0.01 &  0.748$\pm$0.02 &  0.743$\pm$0.02 &  0.694$\pm$0.03 &  0.505$\pm$0.01 &   0.49$\pm$0.01 &  0.553$\pm$0.02 &  0.242$\pm$0.01 &  0.255$\pm$0.01 \\
    & DS &  0.847$\pm$0.01 &  0.823$\pm$0.02 &  0.798$\pm$0.01 &  0.671$\pm$0.05 &  0.596$\pm$0.04 &  0.543$\pm$0.03 &    0.47$\pm$0.1 &  0.382$\pm$0.05 &  0.364$\pm$0.06 &  0.898$\pm$0.02 &  0.848$\pm$0.02 &  0.811$\pm$0.02 &  0.788$\pm$0.06 &  0.638$\pm$0.05 &  0.581$\pm$0.04 &  0.656$\pm$0.11 &  0.408$\pm$0.12 &  0.365$\pm$0.12 &  0.944$\pm$0.02 &  0.846$\pm$0.04 &  0.766$\pm$0.02 &  0.898$\pm$0.12 &   0.659$\pm$0.1 &  0.528$\pm$0.03 &  0.723$\pm$0.14 &  0.466$\pm$0.09 &   0.272$\pm$0.1 \\
    & EBCC &  0.846$\pm$0.01 &  0.829$\pm$0.02 &  0.807$\pm$0.01 &  0.655$\pm$0.05 &  0.582$\pm$0.03 &  0.538$\pm$0.04 &  0.418$\pm$0.11 &   0.31$\pm$0.03 &  0.282$\pm$0.04 &  0.876$\pm$0.03 &   0.84$\pm$0.02 &  0.805$\pm$0.02 &  0.757$\pm$0.06 &  0.589$\pm$0.05 &  0.523$\pm$0.03 &  0.593$\pm$0.15 &  0.286$\pm$0.05 &  0.232$\pm$0.04 &  0.859$\pm$0.04 &  0.767$\pm$0.02 &  0.746$\pm$0.02 &  0.704$\pm$0.09 &  0.512$\pm$0.02 &   0.49$\pm$0.01 &  0.712$\pm$0.09 &  0.263$\pm$0.07 &  0.245$\pm$0.02 \\
    & GLAD &  0.818$\pm$0.01 &  0.777$\pm$0.02 &  0.738$\pm$0.01 &  0.626$\pm$0.02 &  0.558$\pm$0.02 &  0.498$\pm$0.01 &  0.437$\pm$0.02 &  0.346$\pm$0.01 &   0.28$\pm$0.01 &  0.837$\pm$0.01 &  0.793$\pm$0.01 &   0.76$\pm$0.02 &  0.673$\pm$0.01 &  0.577$\pm$0.02 &  0.516$\pm$0.01 &  0.516$\pm$0.02 &  0.359$\pm$0.01 &  0.266$\pm$0.01 &  0.851$\pm$0.01 &  0.783$\pm$0.01 &  0.745$\pm$0.02 &  0.701$\pm$0.02 &  0.577$\pm$0.01 &  0.498$\pm$0.01 &  0.548$\pm$0.02 &  0.353$\pm$0.02 &  0.266$\pm$0.01 \\
    & LFC &  0.852$\pm$0.01 &  0.836$\pm$0.02 &   0.81$\pm$0.01 &  0.686$\pm$0.05 &  0.615$\pm$0.03 &  0.558$\pm$0.04 &     0.5$\pm$0.1 &  0.421$\pm$0.07 &  0.383$\pm$0.06 &   0.91$\pm$0.02 &  0.896$\pm$0.02 &  0.865$\pm$0.02 &  0.856$\pm$0.07 &  0.686$\pm$0.06 &  0.662$\pm$0.04 &  0.726$\pm$0.14 &  0.476$\pm$0.11 &   0.382$\pm$0.1 &  0.954$\pm$0.02 &  0.913$\pm$0.03 &  0.859$\pm$0.04 &  0.966$\pm$0.04 &  0.738$\pm$0.09 &  0.604$\pm$0.05 &    0.84$\pm$0.1 &  0.582$\pm$0.12 &   0.321$\pm$0.1 \\
    & MV &  0.847$\pm$0.01 &  0.794$\pm$0.02 &  0.722$\pm$0.02 &  0.694$\pm$0.02 &  0.594$\pm$0.01 &  0.501$\pm$0.02 &  0.532$\pm$0.04 &  0.385$\pm$0.01 &  0.291$\pm$0.02 &  0.855$\pm$0.01 &  0.804$\pm$0.02 &  0.759$\pm$0.02 &  0.709$\pm$0.02 &    0.6$\pm$0.01 &   0.52$\pm$0.01 &  0.561$\pm$0.02 &  0.394$\pm$0.01 &  0.277$\pm$0.01 &  0.865$\pm$0.01 &  0.791$\pm$0.01 &  0.746$\pm$0.01 &   0.73$\pm$0.02 &  0.592$\pm$0.01 &  0.504$\pm$0.02 &  0.585$\pm$0.02 &  0.377$\pm$0.02 &  0.273$\pm$0.01 \\
    & SURF &  0.962$\pm$0.01 &  0.936$\pm$0.01 &  0.857$\pm$0.01 &  0.968$\pm$0.01 &  0.954$\pm$0.01 &  0.626$\pm$0.04 &  0.901$\pm$0.02 &  0.938$\pm$0.01 &  0.399$\pm$0.04 &   0.997$\pm$0.0 &   0.998$\pm$0.0 &  0.948$\pm$0.11 &   0.998$\pm$0.0 &   0.998$\pm$0.0 &  0.982$\pm$0.04 &  0.966$\pm$0.02 &   0.987$\pm$0.0 &  0.929$\pm$0.08 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.896$\pm$0.13 &     1.0$\pm$0.0 &     1.0$\pm$0.0 &  0.974$\pm$0.06 &   0.995$\pm$0.0 &   0.998$\pm$0.0 &  0.951$\pm$0.07 \\
    & ZC &  0.818$\pm$0.01 &  0.769$\pm$0.02 &  0.745$\pm$0.01 &  0.626$\pm$0.02 &  0.554$\pm$0.02 &   0.49$\pm$0.01 &   0.44$\pm$0.03 &  0.338$\pm$0.02 &  0.261$\pm$0.02 &  0.837$\pm$0.01 &  0.782$\pm$0.02 &  0.758$\pm$0.02 &  0.674$\pm$0.01 &  0.566$\pm$0.02 &  0.507$\pm$0.01 &  0.526$\pm$0.02 &  0.342$\pm$0.02 &   0.25$\pm$0.01 &  0.851$\pm$0.01 &  0.772$\pm$0.02 &  0.743$\pm$0.02 &  0.702$\pm$0.02 &  0.568$\pm$0.01 &   0.49$\pm$0.01 &  0.557$\pm$0.02 &  0.332$\pm$0.02 &  0.257$\pm$0.01 \\
    & iBCC &  0.846$\pm$0.01 &   0.83$\pm$0.02 &  0.804$\pm$0.01 &  0.656$\pm$0.05 &  0.583$\pm$0.04 &  0.525$\pm$0.02 &  0.434$\pm$0.08 &  0.295$\pm$0.04 &  0.284$\pm$0.05 &    0.9$\pm$0.02 &  0.898$\pm$0.02 &   0.89$\pm$0.03 &  0.823$\pm$0.08 &  0.669$\pm$0.06 &  0.618$\pm$0.05 &  0.688$\pm$0.16 &  0.404$\pm$0.14 &  0.312$\pm$0.08 &  0.949$\pm$0.02 &  0.907$\pm$0.03 &  0.896$\pm$0.06 &  0.952$\pm$0.05 &  0.734$\pm$0.09 &  0.567$\pm$0.04 &  0.807$\pm$0.06 &  0.547$\pm$0.11 &   0.267$\pm$0.1 \\
0.5 & CATD &  0.746$\pm$0.02 &  0.748$\pm$0.02 &  0.746$\pm$0.01 &  0.498$\pm$0.01 &  0.498$\pm$0.02 &  0.503$\pm$0.03 &  0.252$\pm$0.01 &  0.246$\pm$0.01 &  0.247$\pm$0.02 &  0.751$\pm$0.02 &   0.75$\pm$0.02 &  0.746$\pm$0.02 &  0.501$\pm$0.02 &  0.507$\pm$0.01 &  0.505$\pm$0.01 &  0.255$\pm$0.02 &  0.257$\pm$0.01 &  0.246$\pm$0.01 &  0.757$\pm$0.01 &  0.745$\pm$0.01 &  0.752$\pm$0.02 &  0.505$\pm$0.01 &  0.498$\pm$0.01 &    0.5$\pm$0.01 &   0.25$\pm$0.02 &  0.249$\pm$0.01 &  0.246$\pm$0.01 \\
    & DS &  0.794$\pm$0.02 &  0.782$\pm$0.02 &  0.762$\pm$0.02 &   0.56$\pm$0.04 &  0.532$\pm$0.03 &   0.52$\pm$0.03 &  0.355$\pm$0.06 &   0.29$\pm$0.02 &   0.28$\pm$0.02 &   0.79$\pm$0.03 &  0.772$\pm$0.02 &  0.751$\pm$0.02 &  0.581$\pm$0.05 &  0.541$\pm$0.02 &  0.511$\pm$0.01 &  0.491$\pm$0.12 &  0.403$\pm$0.09 &   0.25$\pm$0.01 &  0.783$\pm$0.02 &  0.756$\pm$0.02 &  0.757$\pm$0.02 &  0.636$\pm$0.06 &  0.519$\pm$0.02 &  0.502$\pm$0.01 &  0.419$\pm$0.07 &  0.361$\pm$0.06 &  0.246$\pm$0.02 \\
    & EBCC &   0.79$\pm$0.02 &   0.78$\pm$0.02 &  0.762$\pm$0.02 &  0.547$\pm$0.03 &  0.526$\pm$0.02 &  0.515$\pm$0.03 &  0.309$\pm$0.05 &  0.264$\pm$0.01 &   0.25$\pm$0.02 &  0.785$\pm$0.03 &   0.77$\pm$0.02 &  0.752$\pm$0.02 &  0.525$\pm$0.03 &  0.512$\pm$0.01 &  0.508$\pm$0.01 &  0.339$\pm$0.05 &  0.258$\pm$0.01 &  0.245$\pm$0.01 &  0.766$\pm$0.01 &  0.748$\pm$0.01 &  0.754$\pm$0.02 &  0.536$\pm$0.03 &  0.498$\pm$0.01 &    0.5$\pm$0.01 &  0.265$\pm$0.04 &  0.249$\pm$0.01 &  0.246$\pm$0.01 \\
    & GLAD &  0.782$\pm$0.02 &  0.766$\pm$0.02 &  0.741$\pm$0.02 &  0.568$\pm$0.01 &  0.532$\pm$0.02 &  0.506$\pm$0.03 &  0.356$\pm$0.01 &  0.292$\pm$0.01 &  0.256$\pm$0.02 &  0.793$\pm$0.02 &  0.764$\pm$0.01 &  0.746$\pm$0.02 &  0.586$\pm$0.02 &  0.534$\pm$0.02 &  0.508$\pm$0.01 &  0.378$\pm$0.02 &  0.301$\pm$0.02 &  0.253$\pm$0.01 &  0.794$\pm$0.01 &  0.757$\pm$0.01 &  0.754$\pm$0.02 &  0.588$\pm$0.01 &   0.52$\pm$0.01 &  0.501$\pm$0.01 &  0.377$\pm$0.02 &  0.282$\pm$0.01 &  0.249$\pm$0.01 \\
    & LFC &  0.798$\pm$0.02 &  0.786$\pm$0.02 &  0.766$\pm$0.02 &  0.572$\pm$0.04 &  0.537$\pm$0.02 &  0.523$\pm$0.03 &  0.379$\pm$0.06 &  0.322$\pm$0.04 &  0.296$\pm$0.03 &  0.798$\pm$0.03 &  0.781$\pm$0.02 &  0.756$\pm$0.01 &  0.628$\pm$0.06 &  0.565$\pm$0.04 &  0.517$\pm$0.01 &  0.549$\pm$0.14 &   0.44$\pm$0.14 &  0.294$\pm$0.05 &  0.794$\pm$0.02 &  0.768$\pm$0.02 &  0.764$\pm$0.02 &   0.69$\pm$0.09 &  0.586$\pm$0.07 &  0.511$\pm$0.01 &  0.517$\pm$0.09 &  0.451$\pm$0.11 &  0.291$\pm$0.08 \\
    & MV &  0.806$\pm$0.02 &  0.776$\pm$0.02 &   0.73$\pm$0.02 &  0.616$\pm$0.02 &  0.556$\pm$0.02 &  0.507$\pm$0.03 &  0.424$\pm$0.02 &  0.324$\pm$0.01 &  0.261$\pm$0.02 &  0.803$\pm$0.02 &  0.768$\pm$0.01 &  0.745$\pm$0.02 &  0.608$\pm$0.01 &  0.549$\pm$0.02 &  0.511$\pm$0.01 &  0.412$\pm$0.02 &  0.321$\pm$0.02 &  0.258$\pm$0.01 &  0.802$\pm$0.01 &  0.762$\pm$0.01 &  0.755$\pm$0.01 &  0.609$\pm$0.01 &  0.528$\pm$0.01 &  0.502$\pm$0.01 &  0.406$\pm$0.02 &  0.294$\pm$0.01 &   0.25$\pm$0.01 \\
    & SURF &  0.936$\pm$0.01 &   0.89$\pm$0.02 &   0.79$\pm$0.02 &  0.937$\pm$0.02 &  0.848$\pm$0.06 &  0.562$\pm$0.03 &  0.864$\pm$0.02 &  0.834$\pm$0.03 &  0.311$\pm$0.03 &   0.992$\pm$0.0 &   0.989$\pm$0.0 &   0.98$\pm$0.01 &  0.984$\pm$0.01 &   0.992$\pm$0.0 &  0.938$\pm$0.06 &  0.924$\pm$0.01 &   0.977$\pm$0.0 &  0.774$\pm$0.07 &   0.999$\pm$0.0 &     1.0$\pm$0.0 &   0.999$\pm$0.0 &   0.998$\pm$0.0 &   0.999$\pm$0.0 &  0.978$\pm$0.05 &  0.965$\pm$0.01 &   0.991$\pm$0.0 &  0.947$\pm$0.06 \\
    & ZC &  0.782$\pm$0.02 &  0.756$\pm$0.02 &  0.746$\pm$0.01 &  0.568$\pm$0.01 &  0.519$\pm$0.02 &  0.504$\pm$0.03 &  0.356$\pm$0.01 &   0.27$\pm$0.01 &  0.248$\pm$0.02 &  0.793$\pm$0.02 &  0.757$\pm$0.02 &  0.746$\pm$0.02 &  0.586$\pm$0.02 &  0.521$\pm$0.02 &  0.505$\pm$0.01 &  0.378$\pm$0.02 &  0.279$\pm$0.01 &  0.247$\pm$0.01 &  0.794$\pm$0.01 &  0.751$\pm$0.01 &  0.753$\pm$0.01 &  0.588$\pm$0.01 &  0.509$\pm$0.01 &    0.5$\pm$0.01 &  0.377$\pm$0.02 &  0.268$\pm$0.01 &  0.246$\pm$0.01 \\
    & iBCC &  0.791$\pm$0.02 &   0.78$\pm$0.02 &  0.762$\pm$0.02 &  0.546$\pm$0.03 &  0.524$\pm$0.02 &  0.514$\pm$0.03 &   0.31$\pm$0.05 &  0.257$\pm$0.01 &  0.249$\pm$0.02 &   0.79$\pm$0.03 &  0.777$\pm$0.02 &  0.755$\pm$0.01 &  0.593$\pm$0.06 &  0.542$\pm$0.03 &  0.512$\pm$0.01 &  0.484$\pm$0.13 &  0.364$\pm$0.08 &  0.247$\pm$0.01 &  0.788$\pm$0.02 &  0.764$\pm$0.02 &  0.763$\pm$0.02 &   0.65$\pm$0.07 &  0.557$\pm$0.06 &  0.504$\pm$0.01 &  0.467$\pm$0.07 &  0.381$\pm$0.09 &  0.259$\pm$0.03 \\
0.6 & CATD &  0.746$\pm$0.01 &  0.741$\pm$0.02 &  0.741$\pm$0.01 &  0.494$\pm$0.01 &  0.498$\pm$0.02 &  0.486$\pm$0.01 &  0.256$\pm$0.01 &  0.256$\pm$0.01 &  0.247$\pm$0.01 &  0.753$\pm$0.02 &  0.746$\pm$0.01 &  0.747$\pm$0.02 &  0.507$\pm$0.01 &  0.502$\pm$0.02 &  0.505$\pm$0.02 &  0.253$\pm$0.01 &  0.246$\pm$0.01 &  0.249$\pm$0.02 &  0.746$\pm$0.01 &  0.754$\pm$0.01 &  0.744$\pm$0.02 &  0.507$\pm$0.01 &  0.495$\pm$0.01 &  0.497$\pm$0.02 &  0.252$\pm$0.01 &  0.245$\pm$0.01 &  0.252$\pm$0.01 \\
    & DS &  0.766$\pm$0.01 &  0.754$\pm$0.02 &  0.748$\pm$0.01 &  0.522$\pm$0.01 &  0.511$\pm$0.02 &  0.493$\pm$0.01 &  0.292$\pm$0.03 &  0.269$\pm$0.01 &  0.253$\pm$0.01 &  0.765$\pm$0.02 &  0.751$\pm$0.01 &  0.748$\pm$0.01 &  0.516$\pm$0.02 &  0.505$\pm$0.02 &  0.507$\pm$0.01 &  0.332$\pm$0.08 &  0.251$\pm$0.01 &  0.251$\pm$0.02 &  0.749$\pm$0.01 &  0.756$\pm$0.01 &  0.745$\pm$0.02 &  0.512$\pm$0.01 &  0.497$\pm$0.01 &  0.498$\pm$0.02 &  0.279$\pm$0.03 &  0.246$\pm$0.01 &  0.252$\pm$0.01 \\
    & EBCC &  0.765$\pm$0.01 &  0.752$\pm$0.02 &  0.748$\pm$0.01 &  0.517$\pm$0.01 &  0.508$\pm$0.02 &  0.491$\pm$0.01 &  0.274$\pm$0.02 &  0.263$\pm$0.01 &   0.25$\pm$0.01 &  0.765$\pm$0.02 &  0.752$\pm$0.01 &  0.749$\pm$0.02 &  0.515$\pm$0.02 &  0.504$\pm$0.02 &  0.507$\pm$0.01 &  0.281$\pm$0.04 &  0.246$\pm$0.01 &   0.25$\pm$0.02 &  0.751$\pm$0.02 &  0.755$\pm$0.01 &  0.745$\pm$0.02 &  0.508$\pm$0.01 &  0.495$\pm$0.01 &  0.497$\pm$0.02 &  0.253$\pm$0.01 &  0.245$\pm$0.01 &  0.252$\pm$0.01 \\
    & GLAD &  0.763$\pm$0.01 &  0.749$\pm$0.02 &  0.741$\pm$0.01 &  0.527$\pm$0.01 &  0.513$\pm$0.02 &  0.489$\pm$0.02 &  0.304$\pm$0.01 &  0.276$\pm$0.01 &  0.251$\pm$0.01 &  0.768$\pm$0.02 &   0.75$\pm$0.01 &  0.747$\pm$0.02 &  0.535$\pm$0.01 &  0.511$\pm$0.02 &  0.506$\pm$0.01 &  0.297$\pm$0.01 &  0.257$\pm$0.01 &  0.251$\pm$0.02 &  0.756$\pm$0.01 &  0.756$\pm$0.01 &  0.745$\pm$0.02 &  0.527$\pm$0.01 &  0.499$\pm$0.01 &  0.498$\pm$0.02 &  0.282$\pm$0.01 &   0.25$\pm$0.01 &  0.252$\pm$0.01 \\
    & LFC &  0.767$\pm$0.01 &  0.755$\pm$0.02 &   0.75$\pm$0.02 &  0.524$\pm$0.01 &  0.514$\pm$0.02 &  0.495$\pm$0.01 &  0.306$\pm$0.03 &   0.28$\pm$0.03 &  0.256$\pm$0.01 &  0.767$\pm$0.02 &  0.753$\pm$0.01 &   0.75$\pm$0.02 &  0.518$\pm$0.02 &  0.505$\pm$0.02 &  0.508$\pm$0.02 &  0.433$\pm$0.12 &  0.322$\pm$0.06 &  0.252$\pm$0.02 &   0.75$\pm$0.01 &  0.757$\pm$0.01 &  0.746$\pm$0.02 &  0.514$\pm$0.01 &    0.5$\pm$0.02 &  0.498$\pm$0.02 &  0.408$\pm$0.07 &   0.291$\pm$0.1 &  0.252$\pm$0.01 \\
    & MV &   0.78$\pm$0.01 &  0.757$\pm$0.02 &  0.738$\pm$0.01 &  0.558$\pm$0.01 &  0.526$\pm$0.02 &  0.491$\pm$0.02 &  0.352$\pm$0.02 &  0.296$\pm$0.01 &  0.255$\pm$0.01 &  0.773$\pm$0.02 &  0.754$\pm$0.01 &  0.747$\pm$0.02 &  0.546$\pm$0.02 &  0.516$\pm$0.02 &  0.507$\pm$0.01 &  0.315$\pm$0.01 &  0.264$\pm$0.01 &  0.252$\pm$0.02 &   0.76$\pm$0.01 &  0.758$\pm$0.01 &  0.745$\pm$0.02 &  0.536$\pm$0.01 &  0.502$\pm$0.01 &  0.498$\pm$0.02 &  0.296$\pm$0.01 &  0.254$\pm$0.01 &  0.252$\pm$0.01 \\
    & SURF &  0.892$\pm$0.02 &  0.821$\pm$0.02 &  0.765$\pm$0.02 &  0.866$\pm$0.02 &  0.682$\pm$0.04 &  0.513$\pm$0.02 &  0.801$\pm$0.03 &  0.588$\pm$0.06 &  0.274$\pm$0.02 &  0.975$\pm$0.01 &  0.968$\pm$0.01 &  0.852$\pm$0.04 &  0.927$\pm$0.03 &  0.975$\pm$0.01 &  0.733$\pm$0.08 &  0.889$\pm$0.02 &  0.953$\pm$0.01 &  0.462$\pm$0.07 &   0.996$\pm$0.0 &   0.995$\pm$0.0 &  0.978$\pm$0.02 &   0.98$\pm$0.01 &  0.988$\pm$0.01 &  0.949$\pm$0.05 &  0.918$\pm$0.02 &  0.979$\pm$0.01 &  0.772$\pm$0.14 \\
    & ZC &  0.763$\pm$0.01 &  0.744$\pm$0.02 &  0.741$\pm$0.01 &  0.527$\pm$0.01 &  0.502$\pm$0.02 &  0.487$\pm$0.01 &  0.304$\pm$0.01 &  0.265$\pm$0.01 &  0.248$\pm$0.01 &  0.768$\pm$0.02 &  0.748$\pm$0.01 &  0.747$\pm$0.02 &  0.535$\pm$0.01 &  0.506$\pm$0.02 &  0.506$\pm$0.01 &  0.296$\pm$0.01 &   0.25$\pm$0.01 &  0.249$\pm$0.02 &  0.756$\pm$0.01 &  0.754$\pm$0.01 &  0.744$\pm$0.02 &  0.526$\pm$0.01 &  0.496$\pm$0.01 &  0.497$\pm$0.02 &  0.278$\pm$0.01 &  0.247$\pm$0.01 &  0.252$\pm$0.01 \\
    & iBCC &  0.765$\pm$0.01 &  0.752$\pm$0.02 &  0.748$\pm$0.01 &  0.516$\pm$0.01 &  0.507$\pm$0.02 &  0.491$\pm$0.01 &  0.272$\pm$0.02 &  0.262$\pm$0.01 &  0.249$\pm$0.01 &  0.764$\pm$0.02 &  0.752$\pm$0.01 &   0.75$\pm$0.02 &  0.516$\pm$0.02 &  0.505$\pm$0.02 &  0.507$\pm$0.01 &  0.308$\pm$0.04 &  0.248$\pm$0.01 &   0.25$\pm$0.02 &   0.75$\pm$0.01 &  0.757$\pm$0.01 &  0.746$\pm$0.02 &  0.513$\pm$0.01 &  0.497$\pm$0.01 &  0.498$\pm$0.02 &  0.304$\pm$0.07 &  0.258$\pm$0.05 &  0.252$\pm$0.01 \\
\bottomrule
\end{tabular}
}
